Cluster-Promoting Quantization with Bit-Drop for Minimizing Network Quantization Loss

Network quantization, which aims to reduce the bit-lengths of the network weights and activations, has emerged for their deployments to resource-limited devices. Although recent studies have successfully discretized a full-precision network, they still incur large quantization errors after training, thus giving rise to a significant performance gap between a full-precision network and its quantized counterpart. In this work, we propose a novel quantization method for neural networks, Cluster-Promoting Quantization (CPQ) that finds the optimal quantization grids while naturally encouraging the underlying full-precision weights to gather around those quantization grids cohesively during training. This property of CPQ is thanks to our two main ingredients that enable differentiable quantization: i) the use of the categorical distribution designed by a specific probabilistic parametrization in the forward pass and ii) our proposed multi-class straight-through estimator (STE) in the backward pass. Since our second component, multi-class STE, is intrinsically biased, we additionally propose a new bit-drop technique, DropBits, that revises the standard dropout regularization to randomly drop bits instead of neurons. As a natural extension of DropBits, we further introduce the way of learning heterogeneous quantization levels to find proper bit-length for each layer by imposing an additional regularization on DropBits. We experimentally validate our method on various benchmark datasets and network architectures, and also support a new hypothesis for quantization: learning heterogeneous quantization levels outperforms the case using the same but fixed quantization levels from scratch.

==> ablation.tex <==
\section{Ablation Studies}\label{sec:ablation}

In this section, we demonstrate that SRQ and bit-wise sharing DropBits have its own contribution, none of which is negligible. Experiments on the efficiency of a bit-wise sharing mask compared to endpoints-sharing one are postponed to Appendix. % \textcolor{blue}{Experiments on the efficiency of a bit-wise sharing mask are postponed to Appendix \ref{sec:ablation_mask}.}

\vspace{-0.1cm}
Comparing the third, fifth, and last columns in Table \ref{tab:ablation}, we validate the effectiveness of SRQ and DropBits by gradually adding each piece to RQ quantization protocol in series. Although SRQ underperforms RQ on MNIST, SRQ + DropBits performs much better than RQ by introducing quantization noise, which has a regularization effect. Furthermore, DropBits is still well activated to improve generalization even in the case that SRQ much outperforms RQ on CIFAR-10. By observing that SRQ surpasses RQ on CIFAR-10, SRQ appears more suitable for classification tasks on large-scale datasets than RQ, which is an important and powerful feature in a timely manner because recent datasets for deep learning become larger and larger in these days. As a result, DropBits does fit well with SRQ. % in a quantization method by imposing simple binary masks on grid points.

To verify the regularization effect of DropBits on other quantization methods further, we apply DropBits to RQ. Unfortunately, it is not able to reproduce the results of RQ in 2-bit, which makes us apply DropBits to only 3-bit and 4-bit RQ models. Comparing the third and fourth columns in Table \ref{tab:ablation}, DropBits enhances the performance of all RQ models, even including the 4-bit RQ model on MNIST which already surpasses the full-precision model. We therefore argue that DropBits performs well with any quantizer as a regularizer.

\begin{table}[t]
    \vskip -7pt 
	\caption{\small Ablation study for the regularization effect of DropBits and the synergy effect through the mixture of SRQ and DropBits, utilizing LeNet-5 on MNIST/VGG-7 on CIFAR-10.}
	\centering
	{\footnotesize
	\setlength\tabcolsep{4pt}
	\resizebox{7.5cm}{!}{
	\begin{tabular}{c|c|cc|ccc}
	\toprule
	Dataset & \makecell{\# Bits \\ W./A.} & RQ & \makecell{RQ + \\ DropBits} & SRQ & \makecell{SRQ + \\DropBits} \\
	\midrule
	& $4/4$ & $0.58$ & $\mathbf{0.56}$ & $0.72$ & $\mathbf{0.53}$ \\
	MNIST & $3/3$ & $0.69$ & $\mathbf{0.64}$ & $0.84$ & $\mathbf{0.58}$ \\
	& $2/2$ & $0.76$ & - & $0.91$ & $\mathbf{0.63}$ \\
	\midrule
	& $4/4$ & $8.43$ & $\mathbf{8.32}$ & $7.27$ & $\mathbf{6.85}$ \\
	CIFAR-10 & $3/3$ & $9.56$ & $\mathbf{8.95}$ & $7.08$ & $\mathbf{6.94}$ \\
	& $2/2$ & $11.75$ & - & $7.68$ & $\mathbf{7.51}$ \\
	\bottomrule
	\end{tabular}
	}
	}
	\vskip -5pt 
	\label{tab:ablation}
\end{table}

\vspace{-0.1cm}

% \begin{table}[t]
% 	\caption{Ablation study for types of DropBits with LeNet-5 and VGG-7 on MNIST and CIFAR-10 datasets repectively.}
% 	\centering
% 	\begin{tabular}{c|cc|cc}
% 		\toprule
% 		& \multicolumn{2}{c|}{MNIST} & \multicolumn{2}{c}{CIFAR-10} \\
% 		\cmidrule(lr){2-5}
% 		\makecell{Bits \\ W/A} & \makecell{SRQ + \\DropBits \\ (endpoints)} & \makecell{SRQ + \\DropBits \\ (bit-wise)} & \makecell{SRQ + \\DropBits \\ (endpoints)} & \makecell{SRQ + \\DropBits \\ (bit-wise)} \\
% 		\midrule
% 		$4/4$ & $0.64$ & $\mathbf{0.53}$ & $7.51$ & $\mathbf{7.51}$ \\
% 		$3/3$ & $0.65$ & $\mathbf{0.58}$ & $\mathbf{6.96}$ & $6.98$\\
% 		$2/2$ & $0.63$ & $\mathbf{0.63}$ & $6.88$ & $\mathbf{6.85}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:dropbits}
% \end{table}

% \begin{table}[t]
% 	\caption{Ablation study for a synergy effect through the mixture of SRQ and DropBits with LeNet-5 and VGG-7 architectures on MNIST and CIFAR-10 datasets.}
% 	\centering
% 	\begin{tabular}{c|c|ccc}
% 		\toprule
% 		Dataset & \makecell{\# Bits \\ Weights/Act.} & RQ ST & SRQ &  \makecell{SRQ + \\ DropBits} \\
% 		\midrule
% 		& $4/4$ & $0.61$ & $0.72$ & $\mathbf{0.53}$ \\
% 		MNIST & $3/3$ & $0.62$ & $0.84$ & $\mathbf{0.58}$ \\
% 		& $2/2$ & $0.63$ & $0.91$ & $\mathbf{0.63}$ \\
% 		\midrule
% 		& $4/4$ & $7.96$ & $7.27$ & $\mathbf{6.85}$ \\
% 		CIFAR-10 & $3/3$ & $8.92$ & $7.08$ & $\mathbf{6.98}$ \\
% 		& $2/2$ & $9.08$ & $7.68$ & $\mathbf{7.51}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:synergy}
% \end{table}

% \begin{table}[t]
% 	\caption{Ablation study for a regularizing effect of Dropbits on RQ based on MNIST and CIFAR-10 datasets.}
% 	\centering
% 	\begin{tabular}{c|c|cc}
% 		\toprule
% 		Dataset & \makecell{\# Bits \\ Weights/Act.} & RQ & \makecell{RQ + \\ DropBits} \\
% 		\midrule
% 		MNIST & $4/4$ & $0.58$ & $\mathbf{0.56}$ \\
% 		& $3/3$ & $0.69$ & $\mathbf{0.64}$ \\
% 		\midrule
% 		CIFAR-10 & $4/4$ & $8.43$ & $\mathbf{8.32}$ \\
% 		& $3/3$ & $9.56$ & $\mathbf{8.95}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:rq_dropbits}
% \end{table}

% \begin{table}[t]
% 	\caption{Ablation study for a regularizing effect of Dropbits on RQ and RQ ST based on MNIST and CIFAR-10 datasets.}
% 	\centering
% 	\begin{tabular}{c|c|cc|cc}
% 		\toprule
% 		Dataset & \makecell{\# Bits \\ Weights/Act.} & RQ & \makecell{RQ + \\ DropBits} & RQ ST & \makecell{RQ ST + \\ DropBits} \\
% 		\midrule
% 		MNIST & $4/4$ & $0.58$ & $\mathbf{0.56}$ & $0.61$ & $\mathbf{0.56}$ \\
% 		& $3/3$ & $0.69$ & $\mathbf{0.64}$ & $0.62$ & $\mathbf{0.61}$\\
% 		\midrule
% 		CIFAR-10 & $4/4$ & $8.43$ & $\mathbf{8.32}$ & 7.96 & - \\
% 		& $3/3$ & $9.56$ & $\mathbf{8.95}$ & $8.92$ & $\mathbf{8.64}$ \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:ablation_vgg}
% \end{table}
